A local resampling trick for focused molecular dynamics

We describe a method that focuses sampling effort on a user-defined selection of a large system, which can lead to substantial decreases in computational effort by speeding up the calculation of nonbonded interactions. A naive approach can lead to incorrect sampling if the selection depends on the configuration in a way that is not accounted for. We avoid this pitfall by introducing appropriate auxiliary variables. This results in an implementation that is closely related to configurational freezing and elastic barrier dynamical freezing. We implement the method and validate that it can be used to supplement conventional molecular dynamics in free energy calculations (absolute hydration and relative binding).

==> attic.tex <==

\subsection{Exact MCMC within local resampling}
\label{section:local_mcmc}

In the following examples, we consider a system consisting of an arbitrary FreeSolv molecule (\texttt{mobley 242480}) in a small box of TIP3P waters (2689 atoms).

The effect of changing MCMC settings can be evaluated cheaply and simply, since (1) the acceptance rate and other properties can be computed by proposing a single step starting from equilibrium samples, (2) soundness is guaranteed for any setting of the parameters, so we can solely focus on efficiency and avoid the difficulty of assessing bias/efficiency trade-offs.

We pre-generate 500 equilibrium samples using the BAOAB Langevin integrator + Monte Carlo barostat, and estimate the acceptance rate and other properties of various MCMC moves by making proposals starting from these samples. 

\subsubsection{Local Random-Walk Metropolis-Hastings}

We computed the acceptance rates of random-walk Metropolis moves with Gaussian proposals, as a function of the proposal standard deviation.
(Note that these results may be impacted by spurious acceptance rates at large enough proposal standard deviations, due to \url{https://github.com/proteneer/timemachine/issues/481}.)

First, we identify two extremes that any local variant would be expected to lie between: proposing a Gaussian perturbation of 1 particle at a time, and proposing Gaussian perturbations of all particles simultaneously, denoted by the dashed lines in Figure \ref{fig:random_walk_mh}.
The acceptance rates of all-particle vs. 1-particle moves are separated by approximately 2 orders of magnitude on this system.
Next, we construct local moves that select a small spherical region of particles, proposing simultaneous Gaussian perturbations of all particles selected from this region.
The region definition is implied as above, with force constant k = 100.0, %[TODO: units?],
and varying restraint radii (0.0, 0.025, 0.05, 0.1, 0.2, 0.4, 0.8 nanometers).
We observe that the acceptance rates of local moves fall between these two extremes, as expected.

\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/mcmc/random_walk_mh.png}
    \caption{\textbf{Acceptance rates of local random-walk Metropolis interpolate between acceptance rates of moving 1 particle and all particles}.}
    \label{fig:random_walk_mh}
\end{figure}

\subsubsection{Local Metropolis-adjusted Langevin algorithm}

Next, we consider local variants of a gradient-informed move, closer to MD, the Metropolis Adjusted Langevin Algorithm (MALA)~\cite{Roberts1996-pk}.
Recall that MALA is a Metropolis-Hastings algorithm that uses the proposal density 
$q_\tau(\mathbf{y} | \mathbf{x}) = \mathcal{N}(\mathbf{y} ; \mu = \xs - \tau \nabla u(x), \sigma = \sqrt{2 \tau})$
, depending on a step size parameter $\tau$.
This proposal can be motivated as a specific time discretization of overdamped Langevin dynamics, and can scale better to high dimensional targets than random walk proposals.

To side-step the considerations in Section \ref{section:exact_vs_approximate}, a slightly different form of the restraint was used: $u_\text{restraint}(r) = k r^2$, with $k$ selected to yield approximately 50 particles in the local region, $k$ = 5.0.
Sweeping over the step size $\tau$, there is a small separation in acceptance rate between global MALA and local MALA, as shown in Figure \ref{fig:mala}, left.

To assess the ``productivity'' of these moves, we compute the expected squared jump distance (ESJD), as shown in Figure \ref{fig:mala}, middle.
%(The average of squared_jump_distance(x, y) * acceptance_probability(x, y) for x drawn from equilibrium, y proposed from .)
Intuitively, this is summing up the squared displacements of all particles per move.
In cases where we may be more interested in the displacements of the specific atoms selected in the local region.
If we were to modify the measure of sampling productivity (based on a priori interest in the moved particles) by dividing the ESJD by the number of particles moved, there may be a small advantage for local moves, as shown in Figure \ref{fig:mala}, right.
%Intuitively, “average squared displacement for selected particles”.
%Assuming the interesting particles are known, this suggests a possible efficiency advantage for the local move.

\begin{figure}
    \centering
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/mala.png}
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/mala_esjd.png}
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/mala_local_esjd.png}
     \caption{\textbf{Acceptance rate and productivity of local Metropolis-adjsuted Langevin algorithm (MALA).}\\
     Left: Local MALA has slightly higher acceptance rate than global MALA.\\
     Middle: Local MALA has lower maximal productivity (as measured by squared jump distance) than global MALA.\\
     Right: Local MALA has higher maximal productivity per particle (as measured by squared jump distance per selected particle) than global MALA.
     }
    \label{fig:mala}
\end{figure}

\subsubsection{Local Hamiltonian Monte Carlo}
Next, we consider local variants of Hamiltonian Monte Carlo (HMC)~\cite{Neal2012-ya}.
HMC proposals depend on two key parameters: step size, and a number of steps per proposal.
We sweep over step sizes between 0.01 fs and 10 fs, and hold the number of steps per proposal fixed at 10.
All other simulation details are the same as for the local MALA example.
Qualitatively, the behavior of local HMC on this system (Figure \ref{fig:hmc}) is similar to the behavior of local MALA on this system.


\begin{figure}
    \centering
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/hmc_accept_rate.png}
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/hmc_esjd.png}
    \includegraphics[width=0.3\columnwidth]{figures/mcmc/hmc_local_esjd.png}
     \caption{\textbf{Acceptance rate and productivity of local Hamiltonian Monte Carlo (HMC).}\\
     Left: Local HMC has slightly higher acceptance rate than global HMC.\\
     Middle: Local HMC has lower maximal productivity (as measured by squared jump distance) than global MALA.\\
     Right: Local HMC has higher maximal productivity per particle (as measured by squared jump distance per selected particle) than global HMC.
     }
    \label{fig:draft_hmc}
\end{figure}



==> attic_ahfe.tex <==
% full section before condensing


% TODO: show some measure of how much reduction in sampling "productivity" this incurs -- autocorrelation time? [of potential energy] run-to-run variability in some examples? ...
A standard~\cite{Matos2017-dl} approach to predict the absolute hydration free energy (AHFE) of a compound is to perform ``staged'' equilibrium simulations.
(Define a sequence of overlapping thermodynamic states (``windows''), where one window has solute-solvent interactions fully turned off and one window has solute-solvent interactions fully turned on. %over the course of the simulations,
Generate equilibrium samples from each window using any appropriate method (MC, MD, replica exchange, ...),
and then estimate the free energy difference between the first and last window using an appropriate estimator (BAR, MBAR, or TI).
When non-neighboring states have much lower overlap than neighboring states, using BAR~\cite{Bennett1976-un} to estimate the free energy between windows performs similarly to MBAR.)

A default equilibrium sampling approach is all-atom MD.
We consider replacing this default approach (``global MD'') with an alternating sequence of local and global MD moves, then assess whether doing so provides AHFE predictions of equivalent precision and accuracy, at possibly lower computational cost.
%in the context of AHFE calculations could reduce wall time computation, while providing equivalent precision and accuracy.

We selected a subset of Freesolv~\cite{Matos2017-dl,Mobley2014-aw} (\url{https://github.com/MobleyLab/FreeSolv/releases/tag/v0.52}) to benchmark AHFE calculations using local moves for AHFE calculations, refer to Appendix \ref{appendix:freesolv_selection} for details.

% TODO add summary of parameterization and reference appendix
For complete simulation details refer to Appendix \ref{appendix:staged_ahfe_details}.

==> attic_smc.tex <==
% while figuring out how to condense this section


\subsubsection{Local sampling within sequential Monte Carlo}
\label{section:adaptive_smc}
% TODO: key point: not mixing and matching local and global MD in this case
% TODO: comment on box size as well

In Section \ref{section:staged_ahfe}, we controlled the number of steps performed, and confirmed that alternating between unadjusted global and local MD moves does not introduce significant bias into staged hydration free energy predictions.
However, it is difficult to assess the impact of including local moves on overall sampling productivity in this setting.

When controlling for the possibly lower productivity of local MD moves, do application-level efficiency gains still remain?
We attempted to assess this within a framework that adjusts the number of sampling steps based on a measure of their productiveness.
One such framework is adaptive sequential Monte Carlo (SMC)~\cite{Suruzhon2022-gt, Everitt2020-do, Dai2022-ke}, where the next $\lambda$ window can be selected based on the current samples and a heuristic that is sensitive to both the problem’s difficulty and the chosen sampling method’s effectiveness.

Recall~\cite{Del_Moral2006-ov, Dai2022-ke} that in sequential Monte Carlo, a population of walkers %(``particles'')
is first drawn from an initial distribution $p_0$, and then gradually updated (and importance-weighted) using a sequence of transition kernels.
%distributions $(p_t)_{t=0}^T$).
%Roughly, the weight of each particle is updated based on the 
%These particles are then importance-weighted and updated using an alternating sequence of steps, which we might refer to as ``propagation'' and ``perturbation''.
% (TODO: cite NCMC)
These transition kernels are often chosen to be MCMC kernels targeting a sequence of distributions $(p_t)_{t=0}^T$, in which case the importance weights are updated by $p_t(x)/p_{t-1}(x)$ (but there is greater flexibility~\cite{Del_Moral2006-ov} in the SMC framework). 
In applications of SMC to molecular simulation, the MCMC kernels are often chosen to be approximate (i.e. unadjusted MD moves), introducing uncontrolled bias.
The bias may be small in practice~\cite{Suruzhon2022-gt, Gill2018-ag} if the sequence of transitions is gradual enough, and if the approximate MCMC kernels are fast-mixing enough.
In the context of an absolute hydration calculation, $p_0$ may correspond to a thermodynamic state where the solvent and solute are non-interacting, and the sequence $p_t$ may gradually introduce their interactions.

The sequence can be chosen in advance, or it can be determined adaptively.
In particular, we use an adaptive sequential Monte Carlo method that selects the next $\lambda$ window based on the ``conditional effective sample size.''~\cite{Everitt2020-do}.
The number of $\lambda$ windows selected by this method will increase both as a function of transformation difficulty and as a function of how poorly mixing the ``propagation'' steps are.

More details are in Appendix \ref{appendix:smc_details}, but note that this adaptive selection:
\begin{enumerate}
    \item Depends on a parameter that governs the precision (chosen arbitrarily as $\beta = 0.95$).
    This controls how much the effective sample size (ESS) is allowed to decrease between one window and the next $\text{ESS}_{t+1} = \beta \text{ESS}_t$.
    \item Introduces additional overhead to each window’s computation, further limiting the achievable speed-up.
    (In addition to MD, we must evaluate energies on all stored snapshots several times at trial values of $\lambda$ while searching for the next $\lambda_t$.)
    % TODO: stop repeating "application-level speed-up" so much
\end{enumerate}

Applying adaptive SMC to absolute hydration free energy prediction, holding all settings fixed except the choice of using 250 local MD steps vs. 250 global MD steps for propagation, we observe comparable predictions on FreeSolv (97\% within 1 kcal/mol of each other), shown in Figure \ref{fig:smc_preds}.
This suggests that the uncontrolled bias associated with using local MD in this setting is small.

Note that that the sampling biases in the context of SMC may be different from the sampling bias that may arise from alternating unadjusted global and local MD moves (which was investigated in Section \ref{subsection:local_with_unadjusted}).
%In alternating global/local moves, the starting conditions are assumed to be equilibrium samples, 
%In SMC there is the additional risk associated with applying approximate MCMC moves to off-equilibrium conformations.

% TODO: de-junk aspect ratio !!
\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/smc/smc_preds.pdf}
    \caption{
    \textbf{Replacing global propagation with local propagation introduces little bias in an adaptive SMC application.}
    [TODO: make square, add other stats]
    97\% within $\pm$ 1 kcal/mol}
    \label{fig:smc_preds}
\end{figure}

% TODO: double-check these numbers
Next, we consider the competing factors of decreased sampler productivity per step, vs. increased computational speed per step.
Adaptation increases the overall number of $\lambda$ windows for local MD compared to global MD (about 10\% on average) in this case, but this is more than compensated by the increased speed per window when using local MD moves (about 30\% on average), resulting in an application-level speed up of about 13\% for local moves of radius = 1 nm, as summarized in Figure \ref{fig:smc_performance}.
% but this varies by molecule

\begin{figure}
    \centering
    \includegraphics[width=0.8 \columnwidth]{figures/smc/smc_comparison_overall.pdf}
    % \includegraphics[width=0.3 \columnwidth]{figures/smc/n_steps_to_converge.pdf}
    % \includegraphics[width=0.3 \columnwidth]{figures/smc/smc_time_per_window.pdf}
    % \includegraphics[width=0.3 \columnwidth]{figures/smc/smc_wall_time.pdf}
    \caption{
    \textbf{Local propagation accelerates an application where differences in sampling productivity are controlled for.}
    Each dot represents a single molecule in FreeSolv.
    Left: Using local propagation (radius = 1 nm) has lower productivity per step, slightly increasing the number of $\lambda$ windows selected by adaptive SMC.
    Middle: However, the time per window is reduced by a larger factor.
    Right: The net effect is a modest application-level speed-up.
    }
    \label{fig:smc_performance}
\end{figure}

% [TODO: also measure speed-up for local moves of radius = 0.5]

% TODO: investigate what happens with small radius: does this limit ligand sampling (consider long chain), or just solvent response...

% TODO: add histogram of sizes of things in FreeSolv (with a vertical line for the chosen radius (diameter?) of the local region restraint

% TODO: comment on (r0, k, temperature) -> effective radius. (at fixed r0, temperature, (k -> effective "fuzziness" or increment relative to r0))

% TODO: investigate larger radius (or randomized radius, [1 nm, 2 nm])

Taken in the context of expected scaling results and preliminary practical scaling (discussed later in Section \ref{section:practical_speed_up}), % TODO: reference benchmarking_local_md figure
a larger speed-up may be expected for applications where the simulation box is larger.

It is also possible that future implementations may achieve greater speed-up by:
(1) tuning other SMC settings such as number of particles (here chosen arbitrarily as 100),
(2) exploiting the additional parallelism exposed in the SMC application (i.e. running the 100 sampling subproblems in parallel within each window, rather than sequentially),
(3) reducing the cost of energy evaluations during adaptation (exploiting the fact that computing $U(\xs, \lambda)$ at fixed $\xs$ but variable $\lambda$ can be cheaper than computing $U(\xs, \lambda)$,
(4) further improvements in time per local MD step,
(5) using a pre-computed reservoir of waterbox samples.

% TODO: also note a negative result -- possibly in the appendix: negligible application-level speed-up when the local radius is small enough, as the number of windows blows up.

% \subsection{Relative hydration free energy}
% \label{section:rhfe}
% % TODO: reivist

% [\textbf{Placeholder: SECTION MAY NOT BE IN FINAL PAPER}: Would like to report small-scale RHFE results, using 1 or a few benzene derivative pairs from FreeSolv. As of April 21, 2023 these are not computed, but these would be a helpful transition from AHFE to RBFE.]
